OpenTracer: A Dynamic Transaction Trace Analyzer for Smart Contract Invariant Generation and Beyond

Smart contracts, self-executing programs on the blockchain, facilitate reliable value exchanges without centralized oversight. Despite the recent focus on dynamic analysis of their transaction histories in both industry and academia, no open-source tool currently offers comprehensive tracking of complete transaction information to extract user-desired data such as invariant-related data. This paper introduces OpenTracer, designed to address this gap. OpenTracer guarantees comprehensive tracking of every execution step, providing complete transaction information. OpenTracer has been employed to analyze 350,800 Ethereum transactions, successfully inferring 23 different types of invariant from predefined templates. The tool is fully open-sourced, serving as a valuable resource for developers and researchers aiming to study transaction behaviors or extract and validate new invariants from transaction traces. The source code of OpenTracer is available at https://github.com/jeffchen006/OpenTracer.

==> sections/applications.tex <==
\section{Applications}

We now explain possible application scenarios for {\name}.



\noindent
\textbf{Dynamic analysis of transaction history of smart contracts.}



\noindent
\textbf{Development of new smart contract invariants.}



\noindent
\textbf{Replacing Archive Nodes for Other Tools.}

Many analysis tool, like TxSpector, requires an archive node, which is expensive to maintain. 

{\name} can be used to replace archive nodes for other tools.


\noindent
\textbf{Checking with static analysis results.}

{\name} can be used to check the results of static analysis tools.




==> sections/background.tex <==
\section{Background}

% In this section, we provide the necessary background for the rest of the paper.

% \subsection{Concepts}

\noindent\textbf{Blockchain} is a distributed and immutable ledger technology that records transactions across multiple nodes in a network. It employs cryptographic techniques to ensure data integrity and consensus algorithms to maintain final consistency across all participating nodes. \noindent\textbf{Smart contracts} are self-executing programs with the terms of the agreement directly written into code. Deployed on blockchains, they are immutable and transparent, enabling trustless transactions without the need for intermediaries. \noindent \textbf{Invariant guards \camera{(also called circuit breakers)}} are runtime checks around contract invariant conditions that shall always hold during contract execution, aiming to secure smart contracts on the fly.

\noindent\textbf{Ethereum Virtual Machine (EVM)}  is the runtime environment for smart contract execution on Ethereum. It is a Turing-complete virtual machine that interprets and executes the bytecode compiled from contracts programmed in a high-level language like Solidity. \noindent\textbf{Gas} is a unit of transaction fee on Ethereum, used to quantify the computational efforts for the execution of EVM operations. It is paid in \textbf{Ether}, the native cryptocurrency of Ethereum.
\noindent\textbf{Externally Owned Account (EOA) and contract account} are two types of accounts on Ethereum. EOAs are owned by normal users only who have the right to send transactions to blockchains, while contract accounts are controlled by the code deployed at a certain blockchain address and its code will be executed when the contract function is invoked. \noindent\textbf{ERC20} is a standard interface for fungible tokens on Ethereum. Almost all valuable tokens on Ethereum are ERC20 tokens.


%Invariants of a smart contract are conditions that always remain true at a certain program location of the contarct. Invariant guards are runtime checks inserted into the smart contract code to ensure that these invariants hold, thereby enhancing the contract's reliability and security.


% \subsection{Smart Contract Vulnerabilities}

%Smart contracts are computer programs running atop blockchains to facilitate the value transfer process among users.
%Smart contract executions are triggered by blockchain transactions sent by external-owned accounts (EOAs)
%and the interoperability between smart contracts fosters a booming DApp ecosystem like DeFis.
%Managing a large sum of digital assets, smart contracts are vulnerable to security attacks which
%may cause significant financial loss.

\noindent \textbf{Common smart contract vulnerabilities} include integer overflow/underflow~\cite{BECoverflow},
reentrancy~\cite{DAOattacks}, dangerous delegatecall~\cite{Paritystolen}, etc.
% For instance, the Parity wallet contract was hacked in 2017 due to a missing protection of the
% delegatecall operation.
% As a result, the attacker captured the wallet ownership and stole 150K ETH which worth \$30M in USD.
\textbf{DeFi vulnerabilities }are smart contract vulnerabilities that are specific to DeFi applications. They are
more subtle to detect and attacks usually involve more sophisticated steps~\cite{zhou2023sok}.
DeFi protocols are major targets for smart contract attacks, which have experienced \$5.53 billion loss
out of the overall \$6.94 billion caused by recent blockchain incidents~\cite{defillama}.

%Especially, with the advent of dencentralized finance application (DeFi), billions of dollars
%worth asset is run by these applications.
%However, according to the hack statistics~\cite{defillama}, as of 12 September 2023, DeFi hacks
%brought 5.53 billion dollars out of the overall 6.94 billion dollars loss in blockchain incidents.



% Well-known DeFi attacks include governance attacks and oracle price manipulation~\cite{werner2022sok, zhou2023sok}.
%To achieve decentralization, DeFi protocols often implement decentralized governance mechanisms
%based on governance tokens used for proposing and voting on protocol upgrades.
%However, once attackers had sufficient amount of governance tokens to execute malicious proposals,
%the security of the whole DeFi protocols is likely undermined.


% For example, to support asset trading, DeFi applications may rely on price oracles, mostly provided by
% Automated Market Makers (AMMs). If an oracle is designed poorly, attackers can manipulate the oracle price: they first use large amounts of funds to create an imbalance in the liquidity pools within an AMM, leading to a price slippage.
% Since the trading within DeFi applications depends on AMM's price, attackers can make a profit by
% buying DeFi's assets with a lower price and reselling them with a higher price.
% Similar attacks include front-running, where a transaction is submitted purposefully to be executed
% before certain pending user transactions and makes a profit with the price gap.


%Back-running~\cite{bibid} and sandwich attacks~\cite{bibid} can be considered variants of this
%attack.
%



==> tables/calltreeOpcodes.tex <==
\begin{table}[!htbp]
    \caption{EVM Opcodes Used to Construct Invocation Tree}
    \label{tab:calltreeOpcodes}
    \scriptsize
    \begin{tabular}{|l|l|}
    \hline
                    & EVM opcodes                                               \\ \hline
    Function Enter & call, callcode, staticcall, delegatecall, create, create2 \\ \hline
    Function Exit  & stop, return, revert, selfdestruct, (out of gas)          \\ \hline
    \end{tabular}
    \vspace{-4mm}
    \end{table}


==> tables/effectiveness.tex <==
\begin{table}[!htbp]
    \scriptsize
	\vspace{-2mm}
    \caption{Summarized Results of Invariants Effectiveness Evaluation.} 
    \vspace{-4mm}
	\label{tab:rq1summary}
    \tabcolsep=0.11cm
    \resizebox{\columnwidth}{!}{
    	\begin{tabular}{|l|lllll|lll|ll|l|ll|ll|llll|llll|}
			\hline
    																& \multicolumn{5}{c|}{AccessControl}                    						& \multicolumn{3}{c|}{TimeLock}  					& \multicolumn{2}{c|}{GasCtrl} 		& \multicolumn{1}{c|}{Re} 	& \multicolumn{2}{c|}{Oracle} 				& \multicolumn{2}{c|}{Storage} 		& \multicolumn{4}{c|}{Money Flow}                   				& \multicolumn{4}{c|}{Data Flow}                 					\\ \hline
    																& \cellcolor[HTML]{D9D9D9}\rot{EOA}  		& \rot{SO} 			& \rot{SM} 			& \rot{OO} 		& \rot{OM} 			& \rot{SB} 			& \cellcolor[HTML]{D9D9D9}\rot{OB} 		& \rot{LU} 			& \cellcolor[HTML]{D9D9D9}\rot{GS}    	& \rot{GC}       	& \rot{RE}         			& \rot{OR}     	& \rot{OD}    				& \rot{TSU}     & \rot{TBU}    		& \rot{TIU} 	& \cellcolor[HTML]{D9D9D9}\rot{TOU} 	& \rot{TIRU} 	& \rot{TORU} 	& \rot{MU} 		& \rot{CVU} 	& \cellcolor[HTML]{D9D9D9}\rot{DFU} 	& \rot{DFL} 						\\ \hline
			\# Contracts Applied(42)   								& \cellcolor[HTML]{D9D9D9}42 		 		& 39  				& 22  				& 39  			& 25  				& 33 				& \cellcolor[HTML]{D9D9D9}33 			& 37  				& \cellcolor[HTML]{D9D9D9}41  			& 41  				& 40 						& 11   			& 11  						& 21  			& 16   				& 34  			& \cellcolor[HTML]{D9D9D9}34  			& 28  			& 28  			& 11  			& 7   			& \cellcolor[HTML]{D9D9D9}33  			& 33  											\\
			\# Contracts Protected(42) 								& \cellcolor[HTML]{D9D9D9}23  				& 6   				& 7   				& 5   			& 9  				& 11 				& \cellcolor[HTML]{D9D9D9}13 			& 12  				& \cellcolor[HTML]{D9D9D9}30  			& 23  				& 2  						& 7    			& 6   						& 8   			& 12   				& 9   			& \cellcolor[HTML]{D9D9D9}22  			& 5   			& 22  			& 1   			& 2   			& \cellcolor[HTML]{D9D9D9}23  			& 1   											\\
			\# \textbf{Hacks Blocked(27)}     						& \cellcolor[HTML]{D9D9D9}\textbf{15}  		& \textbf{4}   		& \textbf{6}   		& \textbf{3}   	& \textbf{8}   		& \textbf{9}  		& \cellcolor[HTML]{D9D9D9}\textbf{11} 	& \textbf{10}  		& \cellcolor[HTML]{D9D9D9}\textbf{18}  	& \textbf{15}  		& \textbf{2}  				& \textbf{5}    & \textbf{4}   				& \textbf{7}    & \textbf{6}    	& \textbf{8}   	& \cellcolor[HTML]{D9D9D9}\textbf{17}  	& \textbf{5}   	& \textbf{15}  	& \textbf{1}   	& \textbf{2}   	& \cellcolor[HTML]{D9D9D9}\textbf{18}  	& \textbf{1}   									\\
			Average FP(\%)             								& \cellcolor[HTML]{D9D9D9}0.2 				& 0.6 				& 1.8  				& 0.5 			& 2.6 				& 0  				& \cellcolor[HTML]{D9D9D9}0  			& 2.4 				& \cellcolor[HTML]{D9D9D9}2.4 			& 2.6 				& 0  						& 22.3 			& 4.6 						& 7.9 			& 12.6				& 0.7 			& \cellcolor[HTML]{D9D9D9}0.4 			& 0.8 			& 1.4  			& 1.5 			& 0.7 			& \cellcolor[HTML]{D9D9D9}1.6 			& 0.9 											\\ \hline
    	\end{tabular}
    }
	\vspace{-4mm}
\end{table}

